Studying Visualization Guidelines According to Grounded Theory

Visualization guidelines, if defined properly, are invaluable to both practical applications and the theoretical foundation of visualization. In this paper, we present a collection of research activities for studying visualization guidelines according to Grounded Theory (GT). We used the discourses at VisGuides, which is an online discussion forum for visualization guidelines, as the main data source for enabling data-driven research processes as advocated by the grounded theory methodology. We devised a categorization scheme focusing on observing how visualization guidelines were featured in different threads and posts at VisGuides, and coded all 248 posts between September 27, 2017 (when VisGuides was first launched) and March 13, 2019. To complement manual categorization and coding, we used text analysis and visualization to help reveal patterns that may have been missed by the manual effort and summary statistics. To facilitate theoretical sampling and negative case analysis, we made an in-depth analysis of the 148 posts (with both questions and replies) related to a student assignment of a visualization course. Inspired by two discussion threads at VisGuides, we conducted two controlled empirical studies to collect further data to validate specific visualization guidelines. Through these activities guided by grounded theory, we have obtained some new findings about visualization guidelines.

==> README <==
Created by Torsten Moeller (vis@cs.sfu.ca), April 6 2004
modified by Steven Bergner and Torsten Moeller, June 30 2006
modified by James Peltier and Torsten Moeller, March 28, 2007
modified by Bernhard Finkbeiner, July 5, 2010
modified by Tobias Isenberg, January 2016
modified by Filip Sadlo, March 2016
modified by Tobias Isenberg, July 2016

This distribution provides a document class for formatting papers according to the specifications for submission to conferences sponsored by the IEEE Visualization & Graphics Technical Committee (VGTC).

Conferences that use the 'journal' document option:
- IEEE Visualization Conference (VIS, incl. InfoVis, SciVis, VAST)
- IEEE Virtual Reality (VR)
- IEEE International Symposium on Mixed and Augmented Reality (ISMAR)

It contains 13 files/directories:

README          - this file
diamondrule.eps - abstract and body separator
diamondrule.pdf - its PDF version
vgtc.cls        - the VGTC class file, which should be placed, somewhere in the TeX search path (or in the local directory)
template.tex    - an example paper
template.bib    - a small bibliography file used by the example
template.pdf    - an example proper pdf output in default journal mode
abbrv-doi*.bst  - four different versions to generate the bibliography including DOI output, with and without hyperref support, with and without narrow rendering of DOIs
makefile        - makefile including bibtex compilation and proper PDF generation
pictures/       - subdirectory with sample images, both in EPS and in direct pixel/vector format

Usage
=====

The template can be used as such (using the established LaTeX environments) by calling pdfLaTeX or LaTex. For Windows-based LaTeX installations you can use, for example, the environment provided by http://www.texniccenter.org/ along with MikTeX (http://miktex.org/). For Uinux-based installations, please use your favorite LaTeX distribution and editing environment or use the makefile following the instructions below.

Use of the Makefile
===================

Prior to "building" a paper please be sure to run

  make clean

This will ensure that the paper is built cleanly each and every time. We suggest to run this command before each new compilation.

To compile the example, run

  make

or manually, if the makefile does not work for you

  latex template
  bibtex template
  latex template
  latex template

If you run 'make' for the first time, a successful compilation will create a file called 'template.pdf'. Please make sure, that its layout is identical to the file 'template-journal.pdf' provided with this package.

The included makefile also allows you to run each step of the process manually.  Below are a list of available options that may be passed to make

 "make clean"
   removes all files that can be generated automatically.

 "make gs7"
   This will perform all functions to build a proper paper using GhostScript 7.

 "make gs8"
   This will perform all functions to build a proper paper using GhostScript 8.

 "make dvi"
   This will process the .tex file and produce a DVI output file.  This
   step may process the .tex file several times to process all references
   and citations.

 "make ps"
   This will process the .tex file and the DVI output and convert it to a
   PostScript file.

 "make pdf"
   This will process the .tex file using pdfTeX/pdflatex to produce a PDF
   file directly (not using a DVI and PostScript file).
   Please make sure that all fonts are embedded.
   You can use pdffonts my_document.pdf to check if they are.
   It is standard in all modern latex distributions.
   If you use eps figures (e.g. R or gnuplot figures) which you convert to
   PDF using epstopdf, do the following:
   Use GL_OPTIONS, a global environment variable for ghostscript:
   export GS_OPTIONS="-dEmbedAllFonts=true -dPDFSETTINGS=/printer"
   # and run
   epstopdf myfile.eps

   See http://bugs.debian.org/cgi-bin/bugreport.cgi?bug=411651 for the
   origin of this solution.


If you have problems with the makefile please notify us with the output of
the errors produced when running make and we will work to figure out the
resolution.


To produce proper pdf output, please use:
  dvips -t letter -Pdownload35 -Ppdf -G0 template.dvi -o template.ps

The "-Ppdf" and "-G0" flags should be specified in that order; reversing
them does not work, and will result in unacceptable results.

The following information is an exerpt from the ACM SIGGRAPH Conference /
Symposium / Workshop Content Formatting Instructions which can be found
here.

 http://www.siggraph.org/publications/instructions/author-instructions.pdf

If you are using version 7.x of GhostScript, please use the following
method of invoking ‘ps2pdf,’ in order to embed all typefaces and ensure
that images are not downsampled or subsampled in the PDF creation process:

 ps2pdf -dCompatibilityLevel=1.3 -dMaxSubsetPct=100 \
        -dSubsetFonts=true -dEmbedAllFonts=true \
        -dAutoFilterColorImages=false -dAutoFilterGrayImages=false \
        -dColorImageFilter=/FlateEncode -dGrayImageFilter=/FlateEncode \
        -dMonoImageFilter=/FlateEncode template.ps template.pdf

If you are using version 8.x of GhostScript, please use this method in
place of the example above:

 ps2pdf -dPDFSETTINGS=/prepress -dCompatibilityLevel=1.3 \
        -dAutoFilterColorImages=false -dAutoFilterGrayImages=false \
        -dColorImageFilter=/FlateEncode -dGrayImageFilter=/FlateEncode \
        -dMonoImageFilter=/FlateEncode template.ps template.pdf

This has been incorporated into the makefile and should no longer be needed
unless you are building the PDF file manually.


==> makefile <==
# This file seems to originate from something called 'the ultimate
# latex makefile' that different authors worked on. Find original
# versions at:
# http://tadek.pietraszek.org/blog/2006/03/24/the-ultimate-latex-makefile/
# (c) by Tadeusz Pietraszek
# http://www.acoustics.hut.fi/u/mairas/UltimateLatexMakefile/ 
# (c) by Matti Airas
#
# This file has been assembled and adjusted by Steven Bergner, Nov 2005
#  - support for multiple sub-texfiles
#  - fixed '=' '#' problem in mingw/msys environment (see E variable)
#  - PS compilation uses VGTC recommended settings
#  - targets restructured to make PDF by default
#
# Call 'make dvi' for minimal compilation, to check for proper latex
# syntax. This can be much faster than a full PDF generation when big
# figures are involved.
#
# Call 'make pdf' for direct compilation to PDF using pdfTeX. Note that this
# requires you to use .pdf files. pdfTeX can not use .ps or .eps graphics.
# use epstopdf to convert such files to .pdf files.
#
#----------------------------------------------------------------------------
#adjust the following for your purpose

#set the a .dvi name that corresponds to your main .tex file
DVIFILES = template.dvi
MAINTEXFILE = $(DVIFILES:.dvi=.tex)
SUBTEXFILES = 
BIBFILES = template.bib

#switch = to # when using ps2pdf in win32 (mingw/msys), i.e. uncomment 2nd line
#E=\=
E=\#

#adjust paper size: letter/a4
PAPERSIZE=letter
PDFLATEXPAPERSIZE="-sPAPERSIZE$E$(PAPERSIZE)"
DVIPSPAPERSIZE=-t $(PAPERSIZE)
#uncomment the following two lines when using option tvcgpapersize
#DVIPSPAPERSIZE=-T 7.875in,10.75in
#PDFLATEXPAPERSIZE=

#----------------------------------------------------------------------------
LATEX = latex
BIBTEX = bibtex
L2H = latex2html
PDFLATEX = ps2pdf
PDFTEX = pdflatex
DVIPS = dvips 

RERUN = "(There were undefined references|Rerun to get (cross-references|the bars) right)"
RERUNBIB = "No file.*\.bbl|Citation.*undefined" 

PSFILES  = $(DVIFILES:.dvi=.ps) 

PDFFILES7 = $(DVIFILES:.dvi=.pdf7) 
PDFFILES8 = $(DVIFILES:.dvi=.pdf8) 

PDFTEXFILES = $(DVIFILES:.dvi=.pdftex)

COPY = if test -r $*.toc; then cp $*.toc $*.toc.bak; fi 
#RM = /usr/bin/rm -f 
RM = rm -f 

all:	msg gs8

msg:
	@echo "  This script defaults to GhostScript 8.  If you are using GhostScipt 7 please type"
	@echo "  make gs7 instead.  If unsure type gs -v from the command line"
	@echo "  To use pdflatex/pdftex, type make pdf"
	@echo ""


pdf:     clean pdftex 

gs7:        clean dvi ps pdf7

gs8:        clean dvi ps pdf8

dvi:           $(DVIFILES)

ps:           $(PSFILES)

pdf7:           $(PDFFILES7)

pdf8:           $(PDFFILES8)

pdftex:         $(PDFTEXFILES)

$(MAINTEXFILE) : $(SUBTEXFILES) $(BIBFILES)

%.dvi:			%.tex
				$(COPY);$(LATEX) $<
				egrep -c $(RERUNBIB) $*.log && ($(BIBTEX) $*;$(COPY);$(LATEX) $<) ; true
				egrep $(RERUN) $*.log && ($(COPY);$(LATEX) $<) ; true
				egrep $(RERUN) $*.log && ($(COPY);$(LATEX) $<) ; true
				if cmp -s $*.toc $*.toc.bak; then . ;else $(LATEX) $< ; fi
				$(RM) $*.toc.bak
# Display relevant warnings
				egrep -i "(Reference|Citation).*undefined" $*.log ; true

%.pdftex:			%.tex
				echo "wir sind da"
				$(COPY);$(PDFTEX) $<
				egrep -c $(RERUNBIB) $*.log && ($(BIBTEX) $*;$(COPY);$(PDFTEX) $<) ; true
				egrep $(RERUN) $*.log && ($(COPY);$(PDFTEX) $<) ; true
				egrep $(RERUN) $*.log && ($(COPY);$(PDFTEX) $<) ; true
				if cmp -s $*.toc $*.toc.bak; then . ;else $(PDFTEX) $< ; fi
				$(RM) $*.toc.bak
# Display relevant warnings
				egrep -i "(Reference|Citation).*undefined" $*.log ; true

%.ps:			%.dvi
#				dvips -T 7.875in,10.75in -Ppdf -G0 $< -o $@  #use tvcgpapersize
#				dvips -Ppdf -G0 $< -o $@
				dvips $(DVIPSPAPERSIZE) -Pdownload35 -Ppdf -G0 $< -o $@
#				dvips $< -o $@


%.pdf7:			%.ps
	$(PDFLATEX) \
	$(PDFLATEXPAPERSIZE) \
	"-dMaxSubsetPct$E100" \
	"-dCompatibilityLevel$E1.3" \
	"-dSubsetFonts$Etrue" \
	"-dEmbedAllFonts$Etrue" \
	"-dAutoFilterColorImages$Efalse" \
	"-dAutoFilterGrayImages$Efalse" \
	"-dColorImageFilter$E/FlateEncode" \
	"-dGrayImageFilter$E/FlateEncode" \
	"-dMonoImageFilter$E/FlateEncode" \
	$< template.pdf

#				$(PDFLATEX) $<

%.pdf8:                 %.ps
	$(PDFLATEX) \
	$(PDFLATEXPAPERSIZE) \
	"-dPDFSETTINGS=/prepress" \
	"-dCompatibilityLevel=1.3" \
	"-dAutoFilterColorImages=false" \
	"-dAutoFilterGrayImages=false" \
	"-dColorImageFilter=/FlateEncode" \
	"-dGrayImageFilter=/FlateEncode" \
	"-dMonoImageFilter=/FlateEncode" \
	"-dDownsampleGrayImages=false" \
	"-dDownsampleColorImages=false" \
	$< template.pdf
#                               $(PDFLATEX) $<

# cleans anything that can be re-generated automatically, plus emacs backups
clean: 
				rm -f *.aux *.log *.bbl *.blg *.brf *.cb *.ind *.idx *.ilg	\
				*.inx *.toc *.out $(DVIFILES) $(PSFILES) template.pdf *~

.PHONY : all pdf ps dvi clean $(MAINTEXFILE)


==> sections/opencoding-old.v1.tex <==
\section{Categorization and Coding}
\label{sec:VisGuides}
%\ben{ben, alex draft}
%\newcommand{\xx}{\textcolor{red}{XX}}
%\newcommand{\says}[2]{\textit{``#1''}{(#2)}

VisGuides was launched on September 27, 2017 \cite{Diehl:2018:EuroVis}. There were 238 posts up to March 13, 2019 when we collected the latest data set $D_{20190313}$ for the analysis in this paper. The data set contains discourses on some prevalent topics (e.g., color, interaction, virtual reality (VR), and so on), and contributions from users with many different visualization backgrounds, ranging from undergraduate students to highly-respected visualization experts (e.g., in alphabetic order, Niklas Elmqvist, Stephen Few, Eduard Gr\"{o}ller, Theresa-Marie Rhyne, Bernice Rogowitz, and so on).
One cannot help wonder if this data set would inform some ``theories''.Following the tradition in the field of visualization, we use the terms such as ``research questions'', ``hypotheses'', ``categorization schemes'', and ``findings'' instead of ``theories'' in the following discussions.

In this section, we focus on several holistic research questions about visualization guidelines, including
(i) whether and in which way were guidelines mentioned in the posts,
(ii) which guidelines were mentioned and how did the relevant posts discuss them, and
(iii) how should guidelines be categorized?
As $D_{20190313}$ consists of primarily free texts, any answers about ``whether'', ``in which way'', ``which'', and ``how'' depend critically on the interpretation of the texts. From the perspective of grounded theory, the key to befitting interpretations is a correct categorization and coding.

% This section reports on our open coding from XX forum threads. A thread is a question and its answers. Goal of the our open coding was to better understand the use of guidelines in the forum.

Because VisGuides is a computer-assisted platform, the computer has to some extend provided some categorization schemes and automated coding (or selective coding in a grounded theory term). These include those variables in Table \ref{tab:A1-A8} for coding each post. Clearly, these categorization variables would not be sufficient for supporting our investigation into the aforementioned research questions. 

\paragraph{\textbf{Grounded Theory Process.}} \textcolor{red}{TODO}

\paragraph{\textbf{Variables and Categories.}} \textcolor{red}{TODO}

\paragraph{\textbf{Findings.}} \textcolor{red}{TODO}

\textcolor{red}{CURRENT DRAFT BELOW}

\subsection{Methodology}

Our methodology followed several iterative open coding cycles. First, two of the paper authors started reading a random set of around 5-9 articles and tagging them according to information that could potentially be relevant to our questions. Then, the same two authors discussed possible aspects for tagging such as ``what are questions asking for'', ``how specific are they asking for advice'' or ``which guidelines are mentioned in the threads''. For each aspect, we started to formulate categories that we could use to tag a thread. We then asked a third coder to join and explained our aspects and categories to her. Then, each of the three coders individually coded the same set of 10 threads that received most answers (top-10). After coding, the three coders refined categories in each aspects to accommodate for disagreement and diverging interpretations. Finally, one coder went ahead coding another set of \xx threads.

\subsection{Categories}

Our final coding was divided into six \textit{aspects} (A1-A6), with 2-8 \textit{categories} each. Each thread in the forum was classified for all  aspects. If one of the replies could be classified in a certain category, the thread was classified. Thus, multiple categories per thread were possible and in section x, we report on the statistics \textit{per thread}.

\textbf{A1: Type of Question}---This aspect describes the question and what the question is asking for. We found that most questions either asked for help for a specific visualization problems, wanted to discuss a specific guideline (`Don't replicate the real world'), or asked for guidelines around a specific topic (e.g, 3D visualization).

\begin{itemize}[noitemsep]
    \item \textbf{Guideline seeking:} A question looking for guidelines for a specific topic or problem. For a specific problem, the post-creator does not know a guideline or there are no guidelines. Examples include \xx.
    \item \textbf{Guideline use:} a question looking how to employ a specific guideline or asking how to exactly interpret this guideline.
    \item \textbf{Guideline critique}: a guideline is posted (or referenced) and put into question. This requires some argument, motivation, and reason for questioning the specific guideline.
    \item \textbf{Guideline scope}: a question that asks if a particular guideline is valid in a given case and how to apply the guideline for this specific case.
    \item \textbf{Design choices}: a question that posts a specific piece of visualization, asking the audience for advice on its design. Some questions ask about specific design choices (\says{Are the colors I have chosen alright}{2})
\end{itemize}

\textbf{A2: Type of Advice}---This aspect describes what type of advice was given, posted as answers to a question. We found a great variety in the types of replies and decided to settle on the following ones. A more fine-grained categorization might be possible but is out of scope of this paper as (a) this would require a very detailed investigation of the language used, and (b) would help less to answer our specific hypotheses as stated above.

\begin{itemize}[noitemsep]
    \item \textbf{Guideline}: a reply that states a guideline as answer to the question. For example \xx.
    \item \textbf{Critique}: a reply that states and explains a critique to the guideline in question or uses guidelines to critique an initially posted visualization, example, or guideline. Examples include \xx.
    \item \textbf{Clarification/Elaboration}: a reply that clarifies, elaborates, or defends a previously mentioned guideline. This can include delivering arguments in favor of the guideline or detailing its use and meaning. Examples include \xx.
    \item \textbf{General Discussion:} some replies contained discussions that went beyond an individual guideline while discussing other and often more general topics. One example was \says{To make good design choices, we must understand visual perception: what works for the human brain, what doesn't, and why. We develop this ability through study and practice. Asking questions, as you have, is an essential part of this process.}{Few}. 
    \item \textbf{Suggestion:} a reply that made suggestions to question or proposed solutions to a stated problem. Suggestions were very common and contained suggestions about visual encodings (\says{}{}), tools (\says{[...] use a series of sequential ``single hue'' colors maps [...] in ColorBrewer}{}) visualizations (\says{You should also consider using a glyph}{x})
    \item \textbf{Instructive Question}
    \item \textbf{Statement/Fact}
\end{itemize}

\textbf{A3: Specificity}---This aspect describes how specific an advice was given, independent from the type. 

\begin{itemize}[noitemsep]
    \item \textbf{Specific} advise on how to implement a guideline or how to solve a specific problem such as \says{}{}.
    \item \textbf{General} advise on a guidelines or independent from an actual case such as such as \says{}{}. 
\end{itemize}

\textbf{A4: Evidence}---
\begin{itemize}[noitemsep]
    \item \textbf{Publication} includes any scientific publication or text book published through a process that assures some sort of rigor such as peer review, public opinion, or credible experience. Compared to the other categories for this aspect, \textit{Publications} are both traceable and highly credible. Ideally, each reply would use publications as reference, but lack of publications for making a specific point makes this hard. 
    \item \textbf{Web source} includes blogs and websites of both credible sources (Niklas' blog, ColorBrewer) but also less strict and more popular sources such as \xx. 
    \item \textbf{Discussion} includes any reference to a public discussion in a forum, another thread in VisGuides or on Twitter. 
    \item \textbf{Experience/Opinion} include anything that comes from less referable sources such as a participants opinion or experience. Tracing evidence in these cases is possible, but credibility might be low.
\end{itemize}


\textbf{A5: Guidelines}---

\textbf{A6: Topics}---For each thread, we coded \textit{specific} and \textit{general} visualization topics. 
\begin{itemize}[noitemsep]
    \item \textbf{Specific} topics included those explicitly mentioned in the text. Examples include \textit{use-of-color}, \textit{color-schemes}, \textit{human eye-brain system models}, etc. (For a full list, see \xx.)
    \item \textbf{General} topics include those inferred by the coders and referring to more general topics in visualizations. Examples of general topics include \textit{color}, \textit{perception}, \textit{VR}, \textit{interaction}, \textit{learning}, \textit{visual effects}, \textit{3d-visualization}, \textit{2d-visualization}, \textit{cognitive load}, \textit{spatial-data}, \textit{design}, \textit{readability}, \textit{theory-models}, \textit{labeling} (1), and \textit{design} (2).
\end{itemize}

\textbf{A7: Agreement}
\begin{itemize}
    \item \textbf{Agreement} means that discussion participants agreed on an issue or guideline. 
    \item \textbf{Partial agreement} 
    \item \textbf{N/A}
\end{itemize}





\subsection{Findings}

In terms of grounded theory, this example points out some problems and a solution in visualization:

\begin{itemize}
    \item Common-sense advices seem to be a commonplace, and directly quoting guidelines are not common --- possible reasons: no central repository, no adequate evaluation, so lack of confidence for using them.
    \item Although many advices contain sound insight, and many do not make abstraction or generalization --- possible reasons: lack of confidence for defining them or lack of means for proposing them, discussing them, and evaluating them (i.e., not using the grounded theory methodology)
\end{itemize}




==> sections/opencoding-old.v2.tex <==
\section{Categorization and Coding}
\label{sec:VisGuides}
\ben{ben, alex draft}

%\newcommand{\xx}{\textcolor{red}{XX}}
% \newcommand{\says}[2]{\textit{``#1''}{(#2)}}

This section reports on our open coding from XX forum threads. A thread is a question and its answers. Goal of the our open coding was to better understand the use of guidelines in the forum.

(i) if and in which way guidelines are mentioned in the posts?
(ii) which guidelines are mentioned and how a post argues about them, and?
(iii) if and how guidelines are discussed and disputed in the posts?

\subsection{Research questions}


\subsection{Methodology}

Our methodology followed several iterative open coding cycles. First, two of the paper authors started reading a random set of around 5-9 articles and tagging them according to information that could potentially be relevant to our questions. Then, the same two authors discussed possible aspects for tagging such as ``what are questions asking for'', ``how specific are they asking for advice'' or ``which guidelines are mentioned in the threads''. For each aspect, we started to formulate categories that we could use to tag a thread. We then asked a third coder to join and explained our aspects and categories to her. Then, each of the three coders individually coded the same set of 10 threads that received most answers (top-10). After coding, the three coders refined categories in each aspects to accommodate for disagreement and diverging interpretations. Finally, one coder went ahead coding another set of \xx threads.

\subsection{Categories}

Our final coding was divided into six \textit{aspects} (A1-A6), with 2-8 \textit{categories} each. Each thread in the forum was classified for all  aspects. If one of the replies could be classified in a certain category, the thread was classified. Thus, multiple categories per thread were possible and in section x, we report on the statistics \textit{per thread}.

\textbf{D1: Guideline mentioning:} \textit{Are there any guidelines mentioned in the reply and if so, how explicit is this guideline mentioned?} 

\begin{itemize}[noitemsep]
\item \textbf{Explicit:} A guideline is explicitly formulated with a clear advice what to do. Examples of explicit mentionings include \says{Avoid using visual effects in graphs}{15} and \says{Everything in a graph – all of its objects and their visual attributes – should support the graph’s purpose}{16}). Explicit mentioning can include guidelines that are commonly known (e.g, Sheiderman's mantra), or being formulated so that clear advice follows.
\item \textbf{Indirect:} a guideline is indirectly mentioned by pointing to a reference that contains the guideline. Examples include \says{Chapter 2 of [2] provides you with an application of color for labeling of nominal data and its perceptual properties.}{}. The guideline(s) itself are not mentioned explicitly in the reply and it is up to the reader to find and potentially chose. 
%\item \textbf{Implicit:} a guideline is not stated explicitly (nor is it referenced) but an expert in visualization could carefully infer a guideline. For example \says{Pie charts are difficult for the human eye to correctly perceive.} could be re-formulated into ``Avoid pie charts because they are hard to perceive correctly''. 
\item \textbf{No guideline:} the reply is not mentioning any identifiable guideline. This category includes a long list of posts giving very detailed advice, asking questions and making suggestions. These types of messages are captured by our dimension X.		
\item \textbf{Unclear:} the coder is not certain about whether this reply contains a guideline or not.
\end{itemize}


\textbf{D2. Suggestiveness:} \textit{How strong should the reader adhere to the advise?}. This dimension looks at the specific formulations in the post.

\begin{itemize}[noitemsep]
\item \textbf{Imperative:} advice is formulated to imply strict following. Examples include formulations such as 'must', 'do', 'do not', 'should' such as \says{[...] you should consider whether you really need to simultaneously depict them all in a single static image.}
\item \textbf{Indicative:}  (advice can be followed: may, likely, the easiest way?, could, it would, I would)
\item \textbf{Neutral:} (statements which do not allow to infer any suggestion about what to do and what not to do)
\item \textbf{Not-suggestive/informative:}
\item \textbf{Unclear:}
\end{itemize}




\textbf{3. Conditionality:} How conditional is the advice formulated

\begin{itemize}[noitemsep]
\item \textbf{Conditional-explicit:} advice/guideline is stated with a condition when it is valid/not valid and does so explicitly. The condition is stated explicitly.
\item \textbf{Conditional-implicit:} advice does not tell condition explicitly. The reader cannot tell if the guideline applies to them or not. 
\item \textbf{No condition mentioned:} advice/guideline is stated in a way that does not allow to infer when it is valid or not and if there are cases where a guideline is not valid. If there are conditions, the reader does not know.
\item \textbf{Contextual:} advice/guideline does not allow to be generalized easily from the way it is stated. That means that the only condition that make it true are the specific case
\item \textbf{unclear}
\item \textbf{not-applicable}
\end{itemize}




\textbf{4. Support / Backing:} how to we know that a stated advise/guideline is true?  

\begin{itemize}[noitemsep]
\item \textbf{Example:} example case is given to illustrate guideline
\item \textbf{Discussion:} discusses valid and invalid cases for guideline, aiming to provide pro and contra arguments
\item \textbf{Explanation:} explain why guideline should be valid.
\item \textbf{Scientific Reference:} includes an external reference (we have another dimension to classify those)
\item \textbf{Web reference:}
\item \textbf{Opinion:} states an opinion which does not imply if the advices is proven and how valid it is.
\item \textbf{None:} no justification given, just statementx
\item \textbf{Unclear}
\end{itemize}




\textbf{5. Generalizability:} How general is this guideline with respect to other issues in visualization? 

\begin{itemize}[noitemsep]
\item \textbf{General:} applicable to almost every case in visualization, e.g., visualization design, task scope, and conveys methodological meta knowledge about how to do things in visualization, design, reserarch in general. Advise is not specific to an area within visualization.
\item \textbf{Topic-specific:} applicable to specific cases of data, visualization, tasks, contexts, etc.
\item \textbf{Case-specific:} applicable to only this specific case, 'in your case' but not necessarily to other cases with the same problem.
\item \textbf{unclear}
\end{itemize}

\subsection{Findings}

In terms of grounded theory, this example points out some problems and a solution in visualization:

\begin{itemize}
    \item Common-sense advices seem to be a commonplace, and directly quoting guidelines are not common --- possible reasons: no central repository, no adequate evaluation, so lack of confidence for using them.
    \item Although many advices contain sound insight, and many do not make abstraction or generalization --- possible reasons: lack of confidence for defining them or lack of means for proposing them, discussing them, and evaluating them (i.e., not using the grounded theory methodology)
\end{itemize}




==> sections/opencoding-old.v3.tex <==
\section{Categorization and Coding}
\label{sec:VisGuides}
%\ben{ben, alex draft}
%\newcommand{\xx}{\textcolor{red}{XX}}
\newcommand\perc[1]{\the\numexpr#1*100/217\%}
\newcommand{\says}[1]{\textit{`#1'}}



% This section reports on our open coding from XX forum threads. A thread is a question and its answers. Goal of the our open coding was to better understand the use of guidelines in the forum.

In this section, we focus on several holistic research questions about visualization guidelines, including \textbf{Q1-Q3} stated in Section \ref{sec:Introduction}.

Because VisGuides is a computer-assisted platform, the computer has to some extend provided some categorization schemes and automated coding (or selective coding in a grounded theory term). These include those variables in Table \ref{tab:Computer} in Appendix A for coding each post. Clearly, these categorization variables would not be sufficient for supporting our investigation into the aforementioned research questions. 

\newcommand{\xx}{\textcolor{red}{XX}}

\paragraph{\textbf{The GT Coding Process.}}
%
We used the GT methodology to formulate a categorization scheme for the data set $D_{20190313}$, and used the scheme to code all 248 posts in the data set. Two researchers acted as the main coders with the help of from five other researchers. It took three iterations of \emph{open coding}, \emph{axial coding}, and \emph{selective coding} for us to derive the main categorization scheme with six variables (version 3), which was revised slightly to yield version 4.
The details of our GT coding process can be found in Appendix A.4.

% --------------
\begin{figure}[t]
    \centering
    \includegraphics[width=1\columnwidth]{figures/visguides-charts.pdf}
    \caption{Distribution of the categories of the 248 posts in $D_{20190313}$.}
    \label{fig:catstats}
\end{figure}

\paragraph{\textbf{Variables and Categories.}}
Our GT coding process resulted in a categorization scheme with six variables, which include:
%




Dimensions and categories were applied to reflect the main purpose behind a post. Our final dimensions and categories are as follows, with percentages shown in Fig. \ref{fig:catstats} and relations across categories in Fig. \ref{fig:catpcp} 

\begin{itemize}[noitemsep, leftmargin=*]
    \item \textbf{D1: Main Purpose} captures the main purpose of a post. If the post exhibits more than one purpose, the coder made a judgment about what is the main one. Our categories included
    \textit{Ask-for-advice}~(34\%) in which case a post stated a specific problem or visualization example and asked for advice on that problem or visualization; 
    38\% were classified to \textit{Offer advice} and which replied with some sort of advice; \textit{Discuss guidelines}~(\perc{43}) were posts that discussed a specific guideline, questioning their use or correctness.
    \textit{Seek clarification}~(\perc{9}) referred to posts asking for any clarification with respect to a previous post. Eventually, we categorized posts into \textit{social conversation}~\perc{6}, e.g., those thanking for an advice. 
    
    \item \textbf{D2: Guideline mentioning} describes if and how explicit or implicit a post mentions a guidelines. About 19\% of all posts \textit{direct}ly spelled out a well known guideline such as \textit{`Don't Replicate the Real World'}. \textit{Indirect} (12\%) mentions did not spell out the guideline but instead provided a reference, for example \says{Your visualization satisfies many of Stephen Few’s principles [1]'}. Other posts mentioned guidelines \textit{implicit}ly~(4\%) so that a coder could guess the guideline though it was not spelled out explicitly. Examples include \says{A legend is a great tool to aid any visualisation.} and \says{Pie charts are difficult for the human eye to correctly perceive.}. Almost the majority of posts~(51\%), however, did not mention any guidelines and about 14\% could not be classified with enough certainty by the coders.
    
    \item \textbf{D3: Evidence} describes the level of detail and evidence within a statement. Most of the replies (58\%) contained \textit{detailed} evidence by e.g., mentioning details and laying our opinions. Other statements were found to contain \textit{brief} explanations (35\%) with references that would require the reader to search for the detailed arguments and advice themselves. Only about 6\% of all posts did not contain any evidence at all. 2\% of posts could not be classified (\textit{unclear}). 
    
    \item \textbf{D4: Main Scope} describes the scope of the post with respect to how specific or generic is it. For example, the majority of posts was \textit{case-specific}~(64\%) talking about very specific cases and making it hard to generalize to other problems in visualization. 4\% of posts were classified as \textit{conditional}, giving more general advice but at the same time mentioning a specific scope: \says{I understand that the 3D effect for the bar chart [...] is not helpful. But when a chart has overlapping objects, I wonder if I can use some mild 3D effects [...]}. The other large part (25\%) in our data set were \textit{contextual} posts, i.e., posts talking about more general topics in visualization such as color scales, visual perception, interaction etc. 5\% posts were simpler `thank you' messages and could not be classified under any specific scope. 
    
    \item \textbf{D5: Antithesis} describes the stance of a post with respect to its prior post. For example, while only 8\% of the posts were found to have a \textit{neutral} stance, the vast majority 77\% was found to largely agree with the previous post (\textit{so-far-so-good}). While this category included all the initial posts in a thread, after removing them about XX\% of replies fell in this category. A smaller fraction of posts (14\%) contained major \textit{objections} with respect to a previous post. 1\% of posts could not be classified (\textit{unclear}).
    
    \item \textbf{D6: Conviction} classified posts according to how much an author was insisting on his answer to be carried out. 42\% of all posts were rather \textit{neutral}, while 11\% were found \textit{doubtful}, i.e., including some doubts about a guideline or opinion in a previous post. The largest share of posts were formulated in a \textit{suggestive} way (36\%), suggesting a specific action while about 10\% had an \textit{affirmative} character. One post was categorized \textit{unclear} as it contained a very brief call for clarification.
\end{itemize}

\begin{figure}
    \centering
    \includegraphics[width=1\columnwidth]{figures/pcp.pdf}
    \caption{PCP}
    \label{fig:catpcp}
\end{figure}

\subsection{\textbf{Findings.}} %\textcolor{red}{ben: WIP}

\textbf{Using and discussing guidelines is non-trivial.}
Most posts in the forum were asking for advice on very specific cases and replying to such cases (H1), while directly quoting guidelines is not common. Fewer posts (20.74\%) actually discussed guidelines. While this is largely due to the class assignment (Section XX), discussing guidelines is a complex job. If the goal of an advice is to advice in a specific case, it often is sufficient and pragmatic to link to a guideline, state it, or imply it. Though adapting a guideline to a specific case can sometimes be non-trivial and requires discussion, this does not necessarily require knowing all the evidence and expressing total faith in a guideline. Discussing a guideline, in public and with one's name attached, requires more effort and confidence. Discussing a guideline in depth, requires a broad understanding of the specific area of visualization (color theory, 3D visualization, perception, tasks), especially since most cases stretch across fields. It requires knowledge of the literature and the respective evidence as well as cases and examples in order to provide a critical in-depth discussion about the guideline's scope, limitation and how to correctly apply it. In fact, most of the in-depth discussions in the VisGuides forum come from experts in the field of visualization. 

\textbf{Detail is given, but references are missing.}
Many advice in the forum contained sound insight and detailed explanations about the reasons behind an advice. We think this is very positive given that posting in the forum is voluntary. Most explanations contained examples and explained the reasons behind their advice while in other cases, a brief answer is everything it takes to solve a question. Few posts only contained pointers to scientific references and guidelines (). The most common reference we found was to ColorBrewer (), which can be seen as having quasi-guideline status in the visualization community due to its standardized and evidence-based color scale templates. However, we also found that very few people formulating their own guidelines when giving advice. Many posts do not make abstraction or generalization, especially when answering to posts that mention specific cases (seek-advice, give-advice). We believe formulating guidelines, even for very specific cases, can help building `thinking in guidelines' that go beyond specific advice for a specific case.  

\textbf{A central repository could help building a culture around guidelines.}
Other possible reasons for people refraining from using guidelines might include that there is no central repository on guidelines. Such a repository could help establish agreement and help to popularize guidelines as well as increase confidence in using certain guidelines is undermined by missing evaluations. Ideally, such a repository would come in a structured way and includes formulations, references, possible variations, but most importantly the discussions themselves. While part of our research question was to see if and how agreement about guidelines can be established, we require more data and discussion. Of course, such a repository, in part outlined by Scott-Brown~\cite{Scott-Brown2018Presenting}, would require a culture around guidelines that includes use, formulation, evidencing, scoping, and discussing. 

\textbf{Something about discussions here.} Similar may hold for posing questions about guidelines. A large part of the questions we received in the forum ask for very advice on a specific to a varying degree. Some posts very openly asked for `advice' and if a visualization design could be improved. Others replied in more detail and only a tiny fraction () included a guideline in their question. A much smaller fraction () of questions explicitly asked for discussing a specific guideline. Being able to pose a critical question about a guideline requires a broader understanding and expertise. However, the number of posts asking for advice on guidelines in the case of a specific visualization shows that an easy way to start a discussion is to question the application and interpretation of a guideline in a specific example case. 

\textbf{Towards more data and theories.} In summary, the findings from our open coding provide for some discussion and we found our categorization scheme rooted in Grounded Theory to answer our research questions. To generalize and extend our findings, more data is necessary. Through our iterations, we abandoned some dimensions as we found them to require more discussion and definition and data to be truly `grounded'.







% \textcolor{red}{=======OLD DRAFT BELOW======}

% \subsection{Categories}

% Our final coding was divided into six \textit{aspects} (A1-A6), with 2-8 \textit{categories} each. Each thread in the forum was classified for all  aspects. If one of the replies could be classified in a certain category, the thread was classified. Thus, multiple categories per thread were possible and in section x, we report on the statistics \textit{per thread}.

% \textbf{A1: Type of Question}---This aspect describes the question and what the question is asking for. We found that most questions either asked for help for a specific visualization problems, wanted to discuss a specific guideline (`Don't replicate the real world'), or asked for guidelines around a specific topic (e.g, 3D visualization).

% \begin{itemize}[noitemsep]
%     \item \textbf{Guideline seeking:} A question looking for guidelines for a specific topic or problem. For a specific problem, the post-creator does not know a guideline or there are no guidelines. Examples include \xx.
%     \item \textbf{Guideline use:} a question looking how to employ a specific guideline or asking how to exactly interpret this guideline.
%     \item \textbf{Guideline critique}: a guideline is posted (or referenced) and put into question. This requires some argument, motivation, and reason for questioning the specific guideline.
%     \item \textbf{Guideline scope}: a question that asks if a particular guideline is valid in a given case and how to apply the guideline for this specific case.
%     \item \textbf{Design choices}: a question that posts a specific piece of visualization, asking the audience for advice on its design. Some questions ask about specific design choices (\says{Are the colors I have chosen alright}{2})
% \end{itemize}

% \textbf{A2: Type of Advice}---This aspect describes what type of advice was given, posted as answers to a question. We found a great variety in the types of replies and decided to settle on the following ones. A more fine-grained categorization might be possible but is out of scope of this paper as (a) this would require a very detailed investigation of the language used, and (b) would help less to answer our specific hypotheses as stated above.

% \begin{itemize}[noitemsep]
%     \item \textbf{Guideline}: a reply that states a guideline as answer to the question. For example \xx.
%     \item \textbf{Critique}: a reply that states and explains a critique to the guideline in question or uses guidelines to critique an initially posted visualization, example, or guideline. Examples include \xx.
%     \item \textbf{Clarification/Elaboration}: a reply that clarifies, elaborates, or defends a previously mentioned guideline. This can include delivering arguments in favor of the guideline or detailing its use and meaning. Examples include \xx.
%     \item \textbf{General Discussion:} some replies contained discussions that went beyond an individual guideline while discussing other and often more general topics. One example was \says{To make good design choices, we must understand visual perception: what works for the human brain, what doesn't, and why. We develop this ability through study and practice. Asking questions, as you have, is an essential part of this process.}{Few}. 
%     \item \textbf{Suggestion:} a reply that made suggestions to question or proposed solutions to a stated problem. Suggestions were very common and contained suggestions about visual encodings (\says{}{}), tools (\says{[...] use a series of sequential ``single hue'' colors maps [...] in ColorBrewer}{}) visualizations (\says{You should also consider using a glyph}{x})
%     \item \textbf{Instructive Question}
%     \item \textbf{Statement/Fact}
% \end{itemize}

% \textbf{A3: Specificity}---This aspect describes how specific an advice was given, independent from the type. 

% \begin{itemize}[noitemsep]
%     \item \textbf{Specific} advise on how to implement a guideline or how to solve a specific problem such as \says{}{}.
%     \item \textbf{General} advise on a guidelines or independent from an actual case such as such as \says{}{}. 
% \end{itemize}

% \textbf{A4: Evidence}---
% \begin{itemize}[noitemsep]
%     \item \textbf{Publication} includes any scientific publication or text book published through a process that assures some sort of rigor such as peer review, public opinion, or credible experience. Compared to the other categories for this aspect, \textit{Publications} are both traceable and highly credible. Ideally, each reply would use publications as reference, but lack of publications for making a specific point makes this hard. 
%     \item \textbf{Web source} includes blogs and websites of both credible sources (Niklas' blog, ColorBrewer) but also less strict and more popular sources such as \xx. 
%     \item \textbf{Discussion} includes any reference to a public discussion in a forum, another thread in VisGuides or on Twitter. 
%     \item \textbf{Experience/Opinion} include anything that comes from less referable sources such as a participants opinion or experience. Tracing evidence in these cases is possible, but credibility might be low.
% \end{itemize}


% \textbf{A5: Guidelines}---

% \textbf{A6: Topics}---For each thread, we coded \textit{specific} and \textit{general} visualization topics. 
% \begin{itemize}[noitemsep]
%     \item \textbf{Specific} topics included those explicitly mentioned in the text. Examples include \textit{use-of-color}, \textit{color-schemes}, \textit{human eye-brain system models}, etc. (For a full list, see \xx.)
%     \item \textbf{General} topics include those inferred by the coders and referring to more general topics in visualizations. Examples of general topics include \textit{color}, \textit{perception}, \textit{VR}, \textit{interaction}, \textit{learning}, \textit{visual effects}, \textit{3d-visualization}, \textit{2d-visualization}, \textit{cognitive load}, \textit{spatial-data}, \textit{design}, \textit{readability}, \textit{theory-models}, \textit{labeling} (1), and \textit{design} (2).
% \end{itemize}

% \textbf{A7: Agreement}
% \begin{itemize}
%     \item \textbf{Agreement} means that discussion participants agreed on an issue or guideline. 
%     \item \textbf{Partial agreement} 
%     \item \textbf{N/A}
% \end{itemize}







==> sections/relwork.old.v1.tex <==
\section{Background (0.5-1 page}
\label{sec:RelatedWork}

\ben{Ben to draft.  All to contribute references.}

%%%%%
\subsection{What are guidelines?}

Guidelines have been defined as \textit{a general rule, principle, or piece of advice}~\cite{guidelineoxford} and \textit{information intended to advise people on how something should be done or what something should be}~\cite{guidelinecambridge}. Thus, guidelines serve as guardrails for good practices and to help avoiding pitfalls. Guidelines are practical, focused on action, and possibly lend themselves to a mathematical formalization, e.g., \textit{do X, avoid Y}~\cite{Chen:2017:CGA}. A collection of such related guidelines (e.g., on the topic of using colors in visualization) can inform the development of a conceptual model~\cite{Chen:2017:CGA} (e.g., about color perception in visualization) such as Bertin's visual variables~\cite{bertin1983} or Mackinlay's research on performance for specific data types~\cite{Mackinlay_1986}. 

At the same time, guidelines are never mandatory. Rather, they usually are limited as many of them focus on specific cases. Guidelines even can even contradict each other. Our works aims in surfacing and presenting guidelines in visualization as well as to suggest a way of collecting and analyzing guidelines for visualization

%A recent workshop identified  
%'principles and guidelines' as one of four aspects of theoretical advances in visualization, alongside 'taxonomies and ontologies', 'conceptual models and theories frameworks', 'laws and theoretic systems'~\cite{Chen:2017:CGA}. Or example, Bertin's visual variables~\cite{bertin1983} or  Mackinlay's research on performance for specific data types~\cite{Mackinlay_1986} are higher-level frameworks.

% However, while these theories have huge and well acknowledged practical implications, they do not \textit{prescribe} any specific action for a given case. 
% Guidelines, on the other side, have a prescriptive character, have direct practical implications and help making decisions. 

%%%%%
\subsection{Visualization Guidelines}

Guidelines in visualization (\textit{visualization guidelines}) have been part of the evolution of the visualization discipline since its beginning, with contributions from visual arts, perception, and psychology. Prominent examples of visualization guidelines include 
Sheiderman's Mantra \textit{Overview first, zoom and filter, details on demand}~\cite{shneiderman2003eyes}, 
\textit{`Colormap considered harmful'}~\cite{}, 
\textit{Create the simplest graph that conveys the information you want to convey}~\cite{tufte2001visual}, or 
\textit{Select meaningful axis ranges}~\cite{robbins2012creating}. A range of guidelines can be found in papers that propose guidelines as lessons learned for a particular subject, often resulting from empirical quantitative studies or application case studies. Visualization guidelines can be found for text 
highlighting techniques~\cite{strobelt2016guidelines}, 
the use of multiple views~\cite{wang2000guidelines},
hierarchical visualizations~\cite{elmqvist2010hierarchical}, 
the design of information visualization applications~\cite{carr1999guidelines}, 
the design of charts for publication~\cite{kelleher2011ten}, 
making visualizations memorable~\cite{borkin2016beyond}, 
avoid deception~\cite{jones2011lie,monmonier2018lie}, 
use of embellishment in charts~\cite{bateman2010useful},
for visual analytics~\cite{perer2009integrating}, 
for the use of color~\cite{brewer1994color,brewer1994guidelines,borland2007rainbow,silva2011using} and many more.
\ben{more of these examples here?}

However, there is little previous works that proposes and structures a general overview of guidelines. Examples of guideline collections and surveys include Silva's et al. \cite{silva2011using} collection of  guidelines for the use of color in information visualization;
Brodbeck et al. \cite{brodbeck2009interactive} design guidelines for interactive visualizations; and 
Borgo et al. \cite{borgo2013glyph} guidelines for glyph-based visualizations. 

%Many more guidelines can be found online in a rich set of websites, blogs~\cite{DosandDonts,topten,sixguidelines} . However, many of these 'open' guidelines did not underwent scientific peer-reviewing and might lack references and validation. Moreover, as guidelines are always limited and may be valid only for specific cases, we need a better framework for collecting, communicating, and discussing guidelines~\cite{engelke2018visupply}. 
%%%%%
\subsection{Collecting, Curating, and defining guidelines}

Collection, storage, and definition of guidelines are currently not centrally organized. While many guidelines originate and are written down in from scientific papers based on empirical studies, application case studies, or surveys (see above), others originate from blogs or class-room material such as slides~\cite{DosandDonts,topten,sixguidelines}. Fora are sometimes used to discuss guidelines (for an extensive list or fora see~\cite{engelke2018visupply}). Across these media, Scott-Brown~\cite{Scott-Brown2018Presenting} found guidelines reported as \textit{text}, visual, or automated \textit{decision trees}~\cite{data-to-viz}, \textit{checklists}~\cite{datavischecklist} or design patterns~\cite{bach2018narrative,bach2018design}. Eventually, guidelines could be implemented in the form of concise cheat sheets~\cite{WhichVisualization,betterpresentations}. A comprehensive summary of ``about 550 guidelines'' is provided by Kandogan et al.~\cite{Kandogan_2016}, extracted from books, papers, and blogs. The authors compiled statistical summaries of the guidelines and constructed a three-level hierarchy of concepts, sub-concepts and instances using a grounded theory analysis of guidelines, defining a total of 515 categories such as concepts data, visualization, 
users, insights (including tasks supported and knowledge gained), device (physical aspect of visualization medium), and qualifiers indicating specific qualities and quantities in a guideline.

More structured approaches can be found in medicine, where repositories for guidelines exist that capture about 6000 guidelines~\cite{guidelinesinternational}, while the PLOS and Nature journals feature short summary article tracks including data visualization~\cite{naturemethods,plostensimplerules}. Similarly, Scott-Brown suggests a formal and central storage to visualization, alongside with a unique ID, tags, categories, and relations to other guidelines. To streamline the live-cycle of guidelines, Engelke et al. propose a framework for the curation, discussion, and communication of visualization guidelines~\cite{engelke2018visupply} and which consists of steps such as \textit{collection}, \textit{integration}, \textit{contextualization}, \textit{generalization}, and \textit{guideline definition}. 

%As articulated in \cite{Chen:2017:CGA}, visualization guidelines can provide the taxonomies and ontologies in visualization with keywords and causal relations.
%Each guideline can be mapped to a mathematical conjecture, and it can potentially become a theorem when it is mathematically confirmed.
%A collection of related guidelines (e.g., on the topic of using colors in visualization) can inform the development of a conceptual model (e.g., about color perception in visualization).
Our goal is to present methods to obtain a representative picture of the current landscape of guidelines, to rank the most popular ones in the visualization field, and to obtain insights into how to structure and create `guidelines for guidelines'. For example, a guideline may come in a variety of different formats; it can be stated as an imperative (e.g., xx~\cite{}), a suggestion (e.g., ), a fact or pointer to a piece of empirical knowledge (e.g., \textit{humans can only discriminate around 7 colors}). By openly coding replies in our forum, we are interested in how people express and formalize visualization in general and visualization guidelines in particular. 
We also report on the popularity of guidelines weighting citations, subjective expert reporting, trustworthiness of the resources, among other indicators.

\ben{complete}.

\newpage
